Lessons learned from hyper-parameter tuning for microservice candidate identification

When optimizing software for the cloud, monolithic applications need to be partitioned into many smaller *microservices*. While many tools have been proposed for this task, we warn that the evaluation of those approaches has been incomplete; e.g. minimal prior exploration of hyperparameter optimization. Using a set of open source Java EE applications, we show here that (a) such optimization can significantly improve microservice partitioning; and that (b) an open issue for future work is how to find which optimizer works best for different problems. To facilitate that future work, see [https://github.com/yrahul3910/ase-tuned-mono2micro](https://github.com/yrahul3910/ase-tuned-mono2micro) for a reproduction package for this research.

==> bunch.tex <==
\begin{table*}[t]
    \centering
    \caption{Bunch Results} 
    \label{tab:bunch} { \scriptsize
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{jpetstore}
        \label{tab:bunch:jpetstore}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{BCP [-]}  & untuned & \gray{2.43} & 0.0 & \quart{100.0}{0.0}{99.9} \\
             & random & \gray{2.43} & 0.0 & \quart{100.0}{0.0}{99.9} \\
             & hyperopt & \gray{2.43} & 0.0 & \quart{100.0}{0.0}{99.9} \\
            \midrule 
            \multirow{3}{*}{ICP [-]}  & untuned & \gray{0.48} & 0.0 & \quart{100.0}{0.0}{100.6} \\
             & random & \gray{0.48} & 0.0 & \quart{100.0}{0.0}{100.6} \\
             & hyperopt & \gray{0.48} & 0.0 & \quart{100.0}{0.0}{100.6} \\
            \midrule 
            \multirow{3}{*}{SM [+]}  & untuned & \gray{0.21} & 0.0 & \quart{100.0}{0.0}{101.4} \\
             & random & \gray{0.21} & 0.0 & \quart{100.0}{0.0}{101.4} \\
             & hyperopt & \gray{0.21} & 0.0 & \quart{100.0}{0.0}{101.4} \\
            \midrule 
            \multirow{3}{*}{MQ [+]}  & untuned & \gray{7.95} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & random & \gray{7.95} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & \gray{7.95} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{IFN [-]}  & untuned & \gray{2.64} & 0.0 & \quart{100.0}{0.0}{100.2} \\
             & random & \gray{2.64} & 0.0 & \quart{100.0}{0.0}{100.2} \\
             & hyperopt & \gray{2.64} & 0.0 & \quart{100.0}{0.0}{100.2} \\
            \bottomrule
        \end{tabular}
    \end{subtable} 
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{plants}
        \label{tab:bunch:plants}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{BCP [-]}  & untuned & 2.29 & 0.0 & \quart{90.5}{0.0}{90.5} \\
             & random & \gray{1.75} & 0.1 & \quart{65.9}{4.0}{69.2} \\
             & hyperopt & \gray{1.75} & 0.1 & \quart{65.9}{4.0}{69.2} \\
            \midrule 
            \multirow{3}{*}{ICP [-]}  & untuned & 0.56 & 0.0 & \quart{91.8}{0.0}{92.1} \\
             & random & \gray{0.51} & 0.13 & \quart{76.2}{21.4}{83.9} \\
             & hyperopt & \gray{0.51} & 0.13 & \quart{76.2}{21.4}{83.9} \\
            \midrule 
            \multirow{3}{*}{SM [+]}  & untuned & \gray{0.22} & 0.0 & \quart{90.5}{0.0}{91.3} \\
             & random & 0.17 & 0.0 & \quart{68.0}{0.0}{70.5} \\
             & hyperopt & 0.17 & 0.0 & \quart{68.0}{0.0}{70.5} \\
            \midrule 
            \multirow{3}{*}{MQ [+]}  & untuned & 3.88 & 0.0 & \quart{77.4}{0.0}{77.5} \\
             & random & \gray{4.71} & 0.62 & \quart{83.8}{12.4}{94.1} \\
             & hyperopt & \gray{4.71} & 0.62 & \quart{83.8}{12.4}{94.1} \\
            \midrule 
            \multirow{3}{*}{IFN [-]}  & untuned & 4.71 & 0.0 & \quart{100.0}{0.0}{99.9} \\
             & random & \gray{3.88} & 0.48 & \quart{77.8}{10.2}{82.3} \\
             & hyperopt & \gray{3.88} & 0.48 & \quart{77.8}{10.2}{82.3} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.32\textwidth}
        \centering
        \caption{Summary}
        \label{tab:bunch:summary}
        \begin{tabular}{lll}
            \toprule 
            \textbf{Metric} & \textbf{Treatment} & \textbf{Wins} \\
            \midrule
            \multirow{3}{*}{BCP [-]} & untuned & 2 \barc{50} \\
            & random & 3 \barc{75} \\
            & hyperopt & 3 \barc{75} \\
            \midrule
            \multirow{3}{*}{ICP [-]} & untuned & 2 \barc{50} \\
            & random & 4 \barc{100} \\
            & hyperopt & 4 \barc{100} \\
            \midrule
            \multirow{3}{*}{SM [+]} & untuned & 4 \barc{100} \\
            & random & 2 \barc{50} \\
            & hyperopt & 2 \barc{50} \\
            \midrule 
            \multirow{3}{*}{MQ [+]} & untuned & 3 \barc{75} \\
            & random & 3 \barc{75} \\
            & hyperopt & 3 \barc{75} \\
            \midrule
            \multirow{3}{*}{IFN [-]} & untuned & 2 \barc{50} \\
            & random & 4 \barc{100} \\
            & hyperopt & 4 \barc{100} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{daytrader}
        \label{tab:bunch:daytrader}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{BCP [-]}  & untuned & 1.86 & 0.0 & \quart{100.0}{0.0}{100.1} \\
             & random & \gray{1.75} & 0.1 & \quart{89.7}{5.4}{94.2} \\
             & hyperopt & \gray{1.75} & 0.1 & \quart{89.7}{5.4}{94.2} \\
            \midrule 
            \multirow{3}{*}{ICP [-]}  & untuned & 0.57 & 0.0 & \quart{98.8}{0.0}{98.4} \\
             & random & \gray{0.51} & 0.13 & \quart{80.0}{22.5}{88.1} \\
             & hyperopt & \gray{0.51} & 0.13 & \quart{80.0}{22.5}{88.1} \\
            \midrule 
            \multirow{3}{*}{SM [+]}  & untuned & \gray{0.27} & 0.0 & \quart{100.0}{0.0}{100.4} \\
             & random & 0.17 & 0.0 & \quart{61.0}{0.0}{63.2} \\
             & hyperopt & 0.17 & 0.0 & \quart{61.0}{0.0}{63.2} \\
            \midrule 
            \multirow{3}{*}{MQ [+]}  & untuned & \gray{11.33} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & random & 4.71 & 0.62 & \quart{37.0}{5.5}{41.6} \\
             & hyperopt & 4.71 & 0.62 & \quart{37.0}{5.5}{41.6} \\
            \midrule 
            \multirow{3}{*}{IFN [-]}  & untuned & 4.06 & 0.0 & \quart{98.7}{0.0}{98.8} \\
             & random & \gray{3.88} & 0.48 & \quart{89.2}{11.7}{94.4} \\
             & hyperopt & \gray{3.88} & 0.48 & \quart{89.2}{11.7}{94.4} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{acmeair}
        \label{tab:bunch:acmeair}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{BCP [-]}  & untuned & \gray{1.67} & 0.22 & \quart{81.3}{11.6}{87.9} \\
             & random & 1.75 & 0.1 & \quart{87.7}{5.3}{92.1} \\
             & hyperopt & 1.75 & 0.1 & \quart{87.7}{5.3}{92.1} \\
            \midrule 
            \multirow{3}{*}{ICP [-]}  & untuned & \gray{0.55} & 0.09 & \quart{77.9}{15.2}{92.6} \\
             & random & \gray{0.51} & 0.13 & \quart{77.9}{21.9}{85.9} \\
             & hyperopt & \gray{0.51} & 0.13 & \quart{77.9}{21.9}{85.9} \\
            \midrule 
            \multirow{3}{*}{SM [+]}  & untuned & \gray{0.17} & 0.01 & \quart{91.6}{5.6}{95.0} \\
             & random & \gray{0.17} & 0.0 & \quart{91.6}{0.0}{95.0} \\
             & hyperopt & \gray{0.17} & 0.0 & \quart{91.6}{0.0}{95.0} \\
            \midrule 
            \multirow{3}{*}{MQ [+]}  & untuned & \gray{4.39} & 0.61 & \quart{83.8}{12.2}{87.7} \\
             & random & \gray{4.71} & 0.62 & \quart{83.8}{12.4}{94.1} \\
             & hyperopt & \gray{4.71} & 0.62 & \quart{83.8}{12.4}{94.1} \\
            \midrule 
            \multirow{3}{*}{IFN [-]}  & untuned & \gray{3.88} & 0.27 & \quart{93.5}{6.5}{93.7} \\
             & random & \gray{3.88} & 0.48 & \quart{88.5}{11.6}{93.7} \\
             & hyperopt & \gray{3.88} & 0.48 & \quart{88.5}{11.6}{93.7} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \hfill
    }
\end{table*}

==> cogcn.tex <==
\begin{table*}[t]
    \centering
    \caption{CO-GCN Results} 
    \label{tab:cogcn} { \scriptsize
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{jpetstore}
        \label{tab:cogcn:jpetstore}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP [-] }  & untuned & \gray{1.97} & 0.19 & \quart{53.7}{5.5}{57.4} \\
             & random & 2.68 & 0.28 & \quart{73.4}{8.2}{78.0} \\
             & hyperopt & 2.79 & 0.41 & \quart{74.5}{11.9}{81.2} \\
            \midrule 
            \multirow{3}{*}{   ICP [-] }  & untuned & 0.39 & 0.26 & \quart{32.6}{46.3}{69.5} \\
             & random & 0.2 & 0.11 & \quart{32.4}{19.6}{35.7} \\
             & hyperopt & \gray{0.15} & 0.13 & \quart{12.7}{23.2}{26.7} \\
            \midrule 
            \multirow{3}{*}{   SM [+] }  & untuned & 0.16 & 0.08 & \quart{31.3}{31.2}{62.5} \\
             & random & 0.16 & 0.1 & \quart{47.7}{39.1}{62.5} \\
             & hyperopt & \gray{0.19} & 0.07 & \quart{61.4}{27.3}{74.2} \\
            \midrule 
            \multirow{3}{*}{   MQ [+] }  & untuned & \gray{6.11} & 3.6 & \quart{38.1}{49.2}{83.5} \\
             & random & 4.05 & 0.62 & \quart{51.6}{8.5}{55.3} \\
             & hyperopt & 3.9 & 1.52 & \quart{40.7}{20.8}{53.3} \\
            \midrule 
            \multirow{3}{*}{   IFN [-] }  & untuned & \gray{2.0} & 0.44 & \quart{47.0}{11.6}{52.6} \\
             & random & 2.5 & 1.2 & \quart{57.9}{31.6}{65.8} \\
             & hyperopt & 1.8 & 1.25 & \quart{26.3}{32.9}{47.4} \\
             \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{plants}
        \label{tab:cogcn:plants}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & 2.32 & 1.09 & \quart{45.2}{33.8}{72.0} \\
             & random & 2.66 & 0.63 & \quart{76.4}{19.5}{82.5} \\
             & hyperopt & \gray{1.87} & 0.0 & \quart{58.0}{0.0}{58.0} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & 0.51 & 0.11 & \quart{63.4}{16.4}{76.1} \\
             & random & 0.43 & 0.12 & \quart{52.9}{17.9}{64.2} \\
             & hyperopt & \gray{0.02} & 0.0 & \quart{3.3}{0.0}{3.0} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & 0.19 & 0.07 & \quart{53.4}{26.4}{71.7} \\
             & random & 0.19 & 0.09 & \quart{57.5}{34.0}{71.7} \\
             & hyperopt & \gray{0.27} & 0.0 & \quart{100.0}{0.0}{101.9} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & \gray{3.51} & 0.72 & \quart{65.8}{16.8}{82.0} \\
             & random & 2.91 & 0.15 & \quart{65.5}{3.5}{68.0} \\
             & hyperopt & 1.65 & 0.0 & \quart{38.5}{0.0}{38.6} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 4.5 & 1.75 & \quart{48.1}{26.9}{69.2} \\
             & random & 5.75 & 1.06 & \quart{79.8}{16.3}{88.5} \\
             & hyperopt & \gray{1.0} & 0.0 & \quart{15.4}{0.0}{15.4} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.32\textwidth}
        \centering
        \caption{Summary}
        \label{tab:cogcn:summary}
        \begin{tabular}{lll}
            \toprule 
            \textbf{Metric} & \textbf{Treatment} & \textbf{Wins} \\
            \midrule
            \multirow{3}{*}{BCP [-]} & untuned & 2 \barc{50} \\
            & random & 0 \\
            & hyperopt & 2 \barc{50} \\
            \midrule
            \multirow{3}{*}{ICP [-]} & untuned & 0 \\
            & random & 0 \\
            & hyperopt & 4 \barc{100} \\
            \midrule
            \multirow{3}{*}{SM [+]} & untuned & 0 \\
            & random & 2 \barc{50} \\
            & hyperopt & 2 \barc{50} \\
            \midrule 
            \multirow{3}{*}{MQ [+]} & untuned & 4 \barc{100} \\
            & random & 0 \\
            & hyperopt & 0 \\
            \midrule
            \multirow{3}{*}{IFN [-]} & untuned & 1 \barc{25} \\
            & random & 0 \\
            & hyperopt & 3 \barc{75} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{daytrader}
        \label{tab:cogcn:daytrader}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & \gray{1.02} & 0.15 & \quart{32.3}{5.2}{35.0} \\
             & random & 2.32 & 0.54 & \quart{69.5}{18.5}{79.7} \\
             & hyperopt & 2.18 & 0.46 & \quart{66.7}{15.8}{74.9} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & 0.34 & 0.4 & \quart{1.0}{66.4}{56.5} \\
             & random & 0.14 & 0.12 & \quart{6.1}{19.9}{23.3} \\
             & hyperopt & \gray{0.01} & 0.03 & \quart{0.3}{5.0}{1.7} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & 0.1 & 0.04 & \quart{37.9}{19.0}{47.4} \\
             & random & \gray{0.15} & 0.03 & \quart{60.5}{14.2}{71.1} \\
             & hyperopt & 0.11 & 0.04 & \quart{41.1}{19.0}{52.1} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & \gray{7.99} & 5.76 & \quart{35.9}{55.7}{77.3} \\
             & random & 4.34 & 0.71 & \quart{37.0}{6.9}{42.0} \\
             & hyperopt & 3.99 & 0.67 & \quart{37.8}{6.5}{38.6} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 1.96 & 1.98 & \quart{3.0}{26.1}{25.8} \\
             & random & 3.0 & 2.6 & \quart{18.4}{34.2}{39.5} \\
             & hyperopt & \gray{0.5} & 0.4 & \quart{3.3}{5.3}{6.6} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{acmeair}
        \label{tab:cogcn:acmeair}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & 1.5 & 0.13 & \quart{57.0}{5.1}{59.1} \\
             & random & 1.89 & 0.31 & \quart{69.3}{12.2}{74.4} \\
             & hyperopt & \gray{1.31} & 0.0 & \quart{51.6}{0.0}{51.6} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & 0.58 & 0.2 & \quart{58.3}{30.7}{89.0} \\
             & random & 0.46 & 0.1 & \quart{62.1}{15.3}{70.6} \\
             & hyperopt & \gray{0.0} & 0.0 & \quart{0.0}{0.0}{0.0} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & 0.11 & 0.06 & \quart{44.1}{27.3}{50.0} \\
             & random & \gray{0.15} & 0.03 & \quart{61.6}{13.6}{68.2} \\
             & hyperopt & 0.03 & 0.0 & \quart{12.3}{0.0}{13.6} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & \gray{3.71} & 1.68 & \quart{60.0}{38.2}{84.3} \\
             & random & 3.33 & 0.17 & \quart{73.6}{3.9}{75.6} \\
             & hyperopt & 1.0 & 0.0 & \quart{22.7}{0.0}{22.7} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 3.0 & 0.94 & \quart{50.7}{18.1}{57.7} \\
             & random & 4.4 & 0.8 & \quart{76.9}{15.4}{84.6} \\
             & hyperopt & \gray{0.0} & 0.0 & \quart{0.0}{0.0}{0.0} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \hfill
    }
\end{table*}

==> fosci.tex <==
\begin{table*}[t]
    \centering
    \caption{FoSCI Results} 
    \label{tab:fosci} { \scriptsize
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{jpetstore}
        \label{tab:fosci:jpetstore}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP [-] }  & untuned & 2.57 & 0.43 & \quart{75.7}{13.6}{81.1} \\
             & random & 2.43 & 0.3 & \quart{67.2}{9.5}{76.7} \\
             & hyperopt & \gray{2.04} & 0.0 & \quart{64.3}{0.0}{64.4} \\
            \midrule 
            \multirow{3}{*}{   ICP [-] }  & untuned & 0.66 & 0.22 & \quart{63.9}{26.9}{80.7} \\
             & random & \gray{0.04} & 0.05 & \quart{3.8}{6.1}{4.9} \\
             & hyperopt & 0.57 & 0.0 & \quart{69.2}{0.0}{69.7} \\
            \midrule 
            \multirow{3}{*}{   SM [+] }  & untuned & 0.07 & 0.04 & \quart{27.7}{22.6}{39.5} \\
             & random & \gray{0.12} & 0.04 & \quart{65.1}{22.6}{67.8} \\
             & hyperopt & 0.07 & 0.0 & \quart{37.3}{0.0}{39.5} \\
            \midrule 
            \multirow{3}{*}{   MQ [+] }  & untuned & 2.59 & 0.74 & \quart{59.6}{20.4}{71.3} \\
             & random & 2.0 & 0.66 & \quart{49.4}{18.2}{55.1} \\
             & hyperopt & \gray{3.63} & 0.0 & \quart{100.0}{0.0}{99.9} \\
            \midrule 
            \multirow{3}{*}{   IFN [-] }  & untuned & 5.38 & 1.8 & \quart{54.1}{22.5}{67.2} \\
             & random & \gray{1.0} & 1.33 & \quart{12.5}{16.6}{12.5} \\
             & hyperopt & 3.67 & 0.0 & \quart{45.8}{0.0}{45.9} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{plants}
        \label{tab:fosci:plants}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP [-] }  & untuned & 2.39 & 0.13 & \quart{86.0}{4.8}{88.6} \\
             & random & 2.25 & 0.43 & \quart{74.3}{15.9}{83.4} \\
             & hyperopt & \gray{2.04} & 0.0 & \quart{75.5}{0.0}{75.6} \\
            \midrule 
            \multirow{3}{*}{   ICP [-] }  & untuned & 0.62 & 0.12 & \quart{75.0}{15.0}{77.5} \\
             & random & \gray{0.08} & 0.45 & \quart{4.5}{56.2}{10.0} \\
             & hyperopt & 0.57 & 0.0 & \quart{70.8}{0.0}{71.2} \\
            \midrule 
            \multirow{3}{*}{   SM [+] }  & untuned & 0.03 & 0.05 & \quart{5.6}{28.2}{16.9} \\
             & random & \gray{0.11} & 0.05 & \quart{39.7}{28.2}{62.1} \\
             & hyperopt & 0.07 & 0.0 & \quart{37.3}{0.0}{39.5} \\
            \midrule 
            \multirow{3}{*}{   MQ [+] }  & untuned & 2.89 & 0.51 & \quart{67.0}{14.0}{79.6} \\
             & random & 3.26 & 1.75 & \quart{49.4}{48.2}{89.8} \\
             & hyperopt & \gray{3.63} & 0.0 & \quart{100.0}{0.0}{99.9} \\
            \midrule 
            \multirow{3}{*}{   IFN [-] }  & untuned & 5.29 & 0.99 & \quart{71.5}{16.1}{85.8} \\
             & random & \gray{3.0} & 2.45 & \quart{16.2}{39.7}{48.6} \\
             & hyperopt & 3.67 & 0.0 & \quart{59.5}{0.0}{59.5} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.32\textwidth}
        \centering
        \caption{Summary}
        \label{tab:fosci:summary}
        \begin{tabular}{lll}
            \toprule 
            \textbf{Metric} & \textbf{Treatment} & \textbf{Wins} \\
            \midrule
            \multirow{3}{*}{BCP [-]} & untuned & 0 \\
            & random & 0 \\
            & hyperopt & 4 \barc{100} \\
            \midrule
            \multirow{3}{*}{ICP [-]} & untuned & 0 \\
            & random & 4 \barc{100} \\
            & hyperopt & 0 \\
            \midrule
            \multirow{3}{*}{SM [+]} & untuned & 0 \\
            & random & 4 \barc{100} \\
            & hyperopt & 0 \\
            \midrule 
            \multirow{3}{*}{MQ [+]} & untuned & 0 \\
            & random & 0 \\
            & hyperopt & 4 \barc{100} \\
            \midrule
            \multirow{3}{*}{IFN [-]} & untuned & 0 \\
            & random & 4 \barc{100} \\
            & hyperopt & 0 \\
            \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{daytrader}
        \label{tab:fosci:daytrader}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP [-] }  & untuned & 2.9 & 0.66 & \quart{67.5}{19.3}{84.6} \\
             & random & 2.43 & 0.65 & \quart{57.4}{19.0}{70.9} \\
             & hyperopt & \gray{2.04} & 0.0 & \quart{59.4}{0.0}{59.5} \\
            \midrule 
            \multirow{3}{*}{   ICP [-] }  & untuned & 0.71 & 0.14 & \quart{70.8}{17.0}{86.2} \\
             & random & \gray{0.04} & 0.52 & \quart{0.7}{63.1}{4.9} \\
             & hyperopt & 0.57 & 0.0 & \quart{68.7}{0.0}{69.2} \\
            \midrule 
            \multirow{3}{*}{   SM [+] }  & untuned & 0.07 & 0.06 & \quart{24.2}{33.9}{39.5} \\
             & random & \gray{0.12} & 0.07 & \quart{43.8}{39.5}{67.8} \\
             & hyperopt & 0.07 & 0.0 & \quart{37.3}{0.0}{39.5} \\
            \midrule 
            \multirow{3}{*}{   MQ [+] }  & untuned & 2.96 & 0.59 & \quart{68.0}{16.2}{81.5} \\
             & random & 2.0 & 1.2 & \quart{49.4}{33.0}{55.1} \\
             & hyperopt & \gray{3.63} & 0.0 & \quart{100.0}{0.0}{99.9} \\
            \midrule 
            \multirow{3}{*}{   IFN [-] }  & untuned & 5.38 & 0.94 & \quart{60.0}{12.3}{70.2} \\
             & random & \gray{1.0} & 2.72 & \quart{9.8}{35.5}{13.0} \\
             & hyperopt & 3.67 & 0.0 & \quart{47.8}{0.0}{47.9} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{acmeair}
        \label{tab:fosci:acmeair}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP [-] }  & untuned & 2.54 & 0.7 & \quart{70.1}{22.6}{82.0} \\
             & random & 2.42 & 0.46 & \quart{63.7}{14.9}{78.2} \\
             & hyperopt & \gray{2.04} & 0.0 & \quart{65.8}{0.0}{65.9} \\
            \midrule 
            \multirow{3}{*}{   ICP [-] }  & untuned & 0.63 & 0.2 & \quart{57.3}{24.3}{76.5} \\
             & random & \gray{0.06} & 0.23 & \quart{4.4}{27.9}{7.3} \\
             & hyperopt & 0.57 & 0.0 & \quart{68.7}{0.0}{69.2} \\
            \midrule 
            \multirow{3}{*}{   SM [+] }  & untuned & 0.06 & 0.06 & \quart{25.0}{33.9}{33.9} \\
             & random & \gray{0.12} & 0.05 & \quart{55.9}{28.2}{67.8} \\
             & hyperopt & 0.07 & 0.0 & \quart{37.3}{0.0}{39.5} \\
            \midrule 
            \multirow{3}{*}{   MQ [+] }  & untuned & 2.89 & 0.63 & \quart{67.6}{17.3}{79.6} \\
             & random & 1.8 & 1.1 & \quart{47.1}{30.3}{49.6} \\
             & hyperopt & \gray{3.63} & 0.0 & \quart{100.0}{0.0}{99.9} \\
            \midrule 
            \multirow{3}{*}{   IFN [-] }  & untuned & 4.75 & 1.67 & \quart{46.5}{18.6}{52.8} \\
             & random & \gray{1.5} & 2.28 & \quart{11.1}{25.3}{16.7} \\
             & hyperopt & 3.67 & 0.0 & \quart{40.7}{0.0}{40.8} \\
            \bottomrule
        \end{tabular}
    \end{subtable}
    \hfill
    }
\end{table*}

==> mem.tex <==
\begin{table*}[t]
    \centering
    \caption{MEM Results}
    \label{tab:mem} { \scriptsize
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{jpetstore}
        \label{tab:mem:jpetstore}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & \gray{2.69} & 0.0 & \quart{98.2}{0.0}{98.1} \\
             & random & 2.74 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & 2.74 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & \gray{0.47} & 0.01 & \quart{95.8}{2.1}{98.1} \\
             & random & 0.48 & 0.0 & \quart{100.0}{0.0}{100.2} \\
             & hyperopt & 0.48 & 0.0 & \quart{100.0}{0.0}{100.2} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & \gray{0.23} & 0.0 & \quart{90.1}{0.0}{90.9} \\
             & random & 0.22 & 0.0 & \quart{87.0}{0.0}{87.0} \\
             & hyperopt & 0.22 & 0.0 & \quart{87.0}{0.0}{87.0} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & 3.81 & 0.0 & \quart{83.5}{0.0}{83.5} \\
             & random & \gray{4.56} & 0.0 & \quart{100.0}{0.0}{99.9} \\
             & hyperopt & \gray{4.56} & 0.0 & \quart{100.0}{0.0}{99.9} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 4.5 & 0.12 & \quart{97.2}{2.7}{100.0} \\
             & random & 
             \gray{4.0} & 0.0 & \quart{88.9}{0.0}{88.9} \\
             & hyperopt & \gray{4.0} & 0.0 & \quart{88.9}{0.0}{88.9} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable} 
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{plants}
        \label{tab:mem:plants}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & 2.04 & 0.0 & \quart{54.6}{0.0}{54.6} \\
             & random & 3.74 & 0.0 & \quart{100.0}{0.0}{100.1} \\
             & hyperopt & \gray{2.04} & 0.0 & \quart{54.4}{0.0}{54.6} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & 0.43 & 0.0 & \quart{100.0}{0.0}{100.5} \\
             & random & \gray{0.0} & 0.0 & \quart{0.0}{0.0}{0.0} \\
             & hyperopt & 0.42 & 0.0 & \quart{97.4}{0.0}{98.1} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & 0.21 & 0.0 & \quart{86.0}{0.0}{84.0} \\
             & random & 0.1 & 0.0 & \quart{40.8}{0.0}{40.0} \\
             & hyperopt & \gray{0.25} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & 2.66 & 0.0 & \quart{94.1}{0.0}{94.2} \\
             & random & 1.0 & 0.0 & \quart{35.4}{0.0}{35.4} \\
             & hyperopt & \gray{2.83} & 0.0 & \quart{100.0}{0.0}{100.2} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 4.17 & 0.0 & \quart{83.3}{0.0}{83.4} \\
             & random & \gray{0.0} & 0.0 & \quart{0.0}{0.0}{0.0} \\
             & hyperopt & 5.0 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.32\textwidth}
        \centering
        \caption{Summary}
        \label{tab:mem:summary}
        \begin{tabular}{lll}
            \toprule 
            \textbf{Metric} & \textbf{Treatment} & \textbf{Wins} \\
            \midrule
            \multirow{3}{*}{BCP [-]} & untuned & 3 \barc{75} \\
            & random & 0 \\
            & hyperopt & 1 \barc{25} \\
            \midrule
            \multirow{3}{*}{ICP [-]} & untuned & 2 \barc{50} \\
            & random & 2 \barc{50} \\
            & hyperopt & 0 \\
            \midrule
            \multirow{3}{*}{SM [+]} & untuned & 3 \barc{75} \\
            & random & 0 \\
            & hyperopt & 1 \barc{25} \\
            \midrule 
            \multirow{3}{*}{MQ [+]} & untuned & 1 \barc{25} \\
            & random & 2 \barc{50} \\
            & hyperopt & 4 \barc{100} \\
            \midrule
            \multirow{3}{*}{IFN [-]} & untuned & 1 \barc{25} \\
            & random & 3 \barc{75} \\
            & hyperopt & 1 \barc{25} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{daytrader}
        \label{tab:mem:daytrader}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & \gray{1.94} & 0.32 & \quart{93.2}{16.0}{97.0} \\
             & random & 2.0 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & 2.0 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & \gray{0.38} & 0.11 & \quart{63.7}{18.5}{63.9} \\
             & random & 0.59 & 0.0 & \quart{100.0}{0.0}{99.2} \\
             & hyperopt & 0.59 & 0.0 & \quart{100.0}{0.0}{99.2} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & \gray{0.11} & 0.01 & \quart{91.1}{8.9}{98.2} \\
             & random & 0.09 & 0.0 & \quart{83.0}{0.0}{80.4} \\
             & hyperopt & 0.09 & 0.0 & \quart{83.0}{0.0}{80.4} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & 3.15 & 1.01 & \quart{66.7}{21.3}{66.6} \\
             & random & \gray{4.73} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & \gray{4.73} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & \gray{4.08} & 0.85 & \quart{90.6}{18.9}{90.7} \\
             & random & 4.5 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & 4.5 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \bottomrule
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{acmeair}
        \label{tab:mem:acmeair}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & \gray{1.92} & 0.1 & \quart{60.9}{3.3}{64.1} \\
             & random & 3.0 & 0.0 & \quart{100.0}{0.0}{100.1} \\
             & hyperopt & 2.13 & 0.0 & \quart{71.1}{0.0}{71.1} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & 0.66 & 0.08 & \quart{83.6}{11.6}{95.7} \\
             & random & \gray{0.0} & 0.0 & \quart{0.0}{0.0}{0.0} \\
             & hyperopt & 0.69 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & \gray{0.09} & 0.01 & \quart{89.5}{11.6}{104.7} \\
             & random & 0.07 & 0.0 & \quart{80.2}{0.0}{81.4} \\
             & hyperopt & 0.03 & 0.0 & \quart{30.2}{0.0}{34.9} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & \gray{2.77} & 0.53 & \quart{80.8}{19.1}{100.0} \\
             & random & 1.0 & 0.0 & \quart{36.1}{0.0}{36.1} \\
             & hyperopt & \gray{2.58} & 0.0 & \quart{93.3}{0.0}{93.2} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 4.0 & 0.14 & \quart{96.4}{3.5}{100.0} \\
             & random & \gray{0.0} & 0.0 & \quart{0.0}{0.0}{0.0} \\
             & hyperopt & 4.0 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \hfill
    }
\end{table*}

==> mono2micro.tex <==
\begin{table*}[t]
    \centering
    \caption{mono2micro Results}
    \label{tab:mono2micro} { \scriptsize
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{jpetstore}
        \label{tab:mono2micro:jpetstore}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & 2.95 & 0.0 & \quart{100}{0.0}{100} \\
             & random & \gray{1.67} & 0.0 & \quart{56.6}{0.0}{56.6} \\
             & hyperopt & \gray{1.67} & 0.0 & \quart{56.6}{0.0}{56.6} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & \gray{0.51} & 0.0 & \quart{96.2}{0}{96.2} \\
             & random & 0.53 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & 0.53 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & \gray{0.06} & 0.0 & \quart{100}{0.0}{100} \\
             & random & 0.05 & 0.0 & \quart{83.3}{0.0}{83.3} \\
             & hyperopt & 0.05 & 0.0 & \quart{83.3}{0.0}{83.3} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & 2.82 & 0.0 & \quart{85.7}{0.0}{85.7} \\
             & random & \gray{3.29} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & \gray{3.29} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 9.20 & 0.0 & \quart{97.2}{2.7}{100.0} \\
             & random & 
             \gray{3.77} & 0.0 & \quart{41.0}{0.0}{41.0} \\
             & hyperopt & \gray{3.77} & 0.0 & \quart{41.0}{0.0}{41.0} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable} 
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{plants}
        \label{tab:mono2micro:plants}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & 2.95 & 0.0 & \quart{100}{0.0}{100} \\
             & random & \gray{1.73} & 0.0 & \quart{58.6}{0.0}{58.6} \\
             & hyperopt & \gray{1.73} & 0.0 & \quart{58.6}{0.0}{58.6} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & \gray{0.51} & 0.0 & \quart{81.3}{0.0}{81.3} \\
             & random & 0.63 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & 0.63 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & 0.06 & 0.0 & \quart{60.0}{0.0}{60.0} \\
             & random & \gray{0.10} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & \gray{0.10} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & \gray{2.82} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & random & 2.75 & 0.0 & \quart{97.5}{0.0}{97.5} \\
             & hyperopt & 2.75 & 0.0 & \quart{97.5}{0.0}{97.5} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 9.2 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & random & \gray{5.1} & 0.0 & \quart{55.4}{0.0}{55.4} \\
             & hyperopt & \gray{5.1} & 0.0 & \quart{55.4}{0.0}{55.4} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.32\textwidth}
        \centering
        \caption{Summary}
        \label{tab:mono2micro:summary}
        \begin{tabular}{lll}
            \toprule 
            \textbf{Metric} & \textbf{Treatment} & \textbf{Wins} \\
            \midrule
            \multirow{3}{*}{BCP [-]} & untuned & 0 \\
            & random & 4 \barc{100} \\
            & hyperopt & 4 \barc{100} \\
            \midrule
            \multirow{3}{*}{ICP [-]} & untuned & 4 \barc{100} \\
            & random & 0 \\
            & hyperopt & 0 \\
            \midrule
            \multirow{3}{*}{SM [+]} & untuned & 2 \barc{50} \\
            & random & 3 \barc{75} \\
            & hyperopt & 3 \barc{75} \\
            \midrule 
            \multirow{3}{*}{MQ [+]} & untuned & 1 \barc{25} \\
            & random & 3 \barc{75} \\
            & hyperopt & 3 \barc{75} \\
            \midrule
            \multirow{3}{*}{IFN [-]} & untuned & 1 \barc{25} \\
            & random & 4 \barc{100} \\
            & hyperopt & 4 \barc{100} \\
            \bottomrule \\
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{daytrader}
        \label{tab:mono2micro:daytrader}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} &  \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & 1.58 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & random & \gray{1.4} & 0.0 & \quart{88.6}{0.0}{88.6} \\
             & hyperopt & \gray{1.4} & 0.0 & \quart{88.6}{0.0}{88.6} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & \gray{0.40} & 0.0 & \quart{85.7}{0.0}{85.7} \\
             & random & 0.47 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & 0.47 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & \gray{0.06} & 0.0 & \quart{83.3}{0.0}{83.3} \\
             & random & \gray{0.07} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & \gray{0.07} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & 1.83 & 0.0 & \quart{33.1}{0.0}{33.1} \\
             & random & \gray{5.52} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & \gray{5.52} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & \gray{6.2} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & random & \gray{6.13} & 0.0 & \quart{98.87}{0.0}{98.87} \\
             & hyperopt & \gray{6.13} & 0.0 & \quart{98.87}{0.0}{98.87} \\
            \bottomrule
        \end{tabular}
    \end{subtable}
    \begin{subtable}{0.33\textwidth}
        \centering
        \caption{acmeair}
        \label{tab:mono2micro:acmeair}
        \begin{tabular}{lllll}
            \toprule
            \textbf{Metric} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \textbf{Quartiles} \\
            \midrule
            \multirow{3}{*}{   BCP[-] }  & untuned & 1.58 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & random & \gray{1.04} & 0.0 & \quart{65.8}{0.0}{65.8} \\
             & hyperopt & \gray{1.04} & 0.0 & \quart{65.8}{0.0}{65.8} \\
            \midrule 
            \multirow{3}{*}{   ICP[-] }  & untuned & \gray{0.4} & 0.0 & \quart{66.6}{0.0}{66.6} \\
             & random & 0.59 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & 0.59 & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   SM[+] }  & untuned & 0.06 & 0.0 & \quart{60.0}{0.0}{60.0} \\
             & random & \gray{0.1} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & \gray{0.1} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   MQ[+] }  & untuned & 1.83 & 0.0 & \quart{53.2}{0.0}{53.2} \\
             & random & \gray{3.44} & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & hyperopt & \gray{3.44} & 0.0 & \quart{100.0}{0.0}{100.0} \\
            \midrule 
            \multirow{3}{*}{   IFN[-] }  & untuned & 6.2 & 0.0 & \quart{100.0}{0.0}{100.0} \\
             & random & \gray{3.3} & 0.0 & \quart{53.2}{0.0}{53.2} \\
             & hyperopt & \gray{3.3} & 0.0 & \quart{53.2}{0.0}{53.2} \\
            \bottomrule 
        \end{tabular}
    \end{subtable}
    \hfill
    }
\end{table*}

==> summary.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{mono2micro.png}
        \caption{mono2micro}
        \label{fig:summary:mono2micro}
    \end{subfigure}%
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{cogcn.png}
        \caption{CO-GCN}
        \label{fig:summary:cogcn}
    \end{subfigure}%
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{bunch.png}
        \caption{Bunch}
        \label{fig:summary:bunch}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{mem.png}
        \caption{MEM}
        \label{fig:summary:mem}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fosci.png}
        \caption{FoSCI}
        \label{fig:summary:fosci}
    \end{subfigure}%
    \hfill
    \caption{Comparison of the tuning approaches across datasets for each metric. In each figure, blue represents random, green represents hyperopt, and gray represents a tie.}
    \label{fig:summary}
\end{figure*}
